A General Framework for Modelling Conditional Reasoning -- Preliminary Report

We introduce and investigate here a formalisation for conditionals that allows the definition of a broad class of reasoning systems. This framework covers the most popular kinds of conditional reasoning in logic-based KR: the semantics we propose is appropriate for a structural analysis of those conditionals that do not satisfy closure properties associated to classical logics.

==> macros.tex <==
\usepackage{times}
\usepackage{helvet}
\usepackage{courier}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Used packages:
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{mathtools}
\usepackage{mathrsfs} % manuscript style in math mode
%\usepackage{eucal} % for Euler style mathcal. Alternative: \usepackage[mathcal]{euler}
\usepackage{ifsym}
\usepackage{bbm} % To get |N, |R, Z, use \mathbbm{N}, \mathbbm{R}, \mathbbm{Z}
\usepackage{color}
\usepackage[svgnames]{xcolor}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{tikz} 
\usetikzlibrary{shapes.misc,automata,positioning,arrows}
\usepgflibrary{shapes.arrows} 
\usepackage{dsfont}
\usepackage{url}
%\usepackage{datetime}
\usepackage{setspace}
\usepackage{varioref}
\usepackage{xspace} % adds and removes space after macros: Add \xspace at end of macro
\usepackage{stmaryrd}
\usepackage[ruled,linesnumbered,vlined,scleft]{algorithm2e}
\usepackage{engord}
\usepackage{comment}
\usepackage{pifont}
\usepackage{mathabx} % to get an `O' for obligation in deontic logic with \ovoid
\usepackage{amsmath}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General expressions and commands:

\newcommand{\ie}{\mbox{i.e.}}
\newcommand{\eg}{\mbox{e.g.}}
\newcommand{\cf}{\mbox{cf.}}
\newcommand{\viz}{\mbox{viz.}}
\newcommand{\wrt}{\mbox{w.r.t.}}
\newcommand{\st}{\mbox{s.t.}}
\newcommand{\wolog}{\mbox{w.l.o.g.}}
\newcommand{\etal}{\mbox{et al}}
\newcommand{\myskip}{\smallskip} % space interlines
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical general expressions:  

\newcommand{\qed}{[\textsc{qed}]}%\rule{2mm}{2mm}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\defined}{\ensuremath{\equiv_{\text{def}}}}
\newcommand{\abbrev}{\mathrel{\mathop:}=}
\newcommand{\eqclass}[1]{[#1]} % equivalence class of an element

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem-like environments:

%\theoremstyle{break}
\newtheorem{definition}{Definition}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{theorem}{Theorem}%[section] 
\newtheorem{proposition}{Proposition}%[section]
\newtheorem{corollary}{Corollary}%[section]
\newtheorem{conjecture}{Conjecture}%[section]
\newtheorem{observation}{Observation}%[section]
\newtheorem{claim}{Claim}%[section]
%{\theorembodyfont{\upshape}
\newtheorem{example}{Example}%[section]%}
%{\theoremstyle{plain}\theorembodyfont{\upshape}
\newtheorem{remark}{Remark}%[section]%}
\newenvironment{proof}{\noindent\textbf{Proof:}\null\hfill\null\newline}{\hfill\qed}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computational complexity:

\newcommand{\ptime}{\textsc{P}}
\newcommand{\np}{\textsc{NP}}
\newcommand{\exptime}{\textsc{exptime}}
\newcommand{\pspace}{\textsc{pspace}}
\newcommand{\npcomplete}{\textsc{np-complete}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sets and set operations:

% Set union: \cup, Set intersection: \cap, Set difference: \setminus
\newcommand{\powerset}[1]{\mathscr{P}(#1)} % powerset
\newcommand{\symdiff}{\dotdiv} % symmetric difference

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special sets:

% Language:
\newcommand{\Prp}{\ensuremath{\mathcal{P}}}
\newcommand{\Sig}{\ensuremath{\mathcal{S}}} % a set of atoms, or a signature
\newcommand{\Lang}{\ensuremath{\mathcal{L}}}

% Theories:
\newcommand{\T}{\ensuremath{\mathcal{T}}} % a theory
\newcommand{\KB}{\ensuremath{\mathcal{K}}} % a knowledge base

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Logical connectives and meta-logical basic definitions:

% Logical negation: \lnot, Logical conjunction: \land, Logical disjunction: \lor
\newcommand{\limp}{\rightarrow} % logical implication
\newcommand{\liff}{\leftrightarrow} % biconditional
\newcommand{\lexor}{\oplus} % exclusive or

% Satisfaction, entailment and derivability relations:
\newcommand{\sat}{\Vdash}
\newcommand{\nsat}{\Vdash\hspace{-0.28cm}{/}\hspace{0.1cm}}
\newcommand{\nratcl}{\ratcl\hspace{-0.6cm}{/}\hspace{0.4cm}}
\newcommand{\nprefcl}{\prefcl\hspace{-0.65cm}{/}\hspace{0.45cm}}
\newcommand{\nosat}{\not\Vdash}
\newcommand{\entails}{\models}
\newcommand{\nentails}{\not\entails}
\newcommand{\entailed}{\raisebox{1.1ex}{\rotatebox{180}{$\entails$}}}
\newcommand{\proves}{\vdash}
\newcommand{\nproves}{\not\proves}
\newcommand{\nrat}{\not\ratcl}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Classical Propositional Logic:

\newcommand{\fml}{\ensuremath{\varphi}} % a classical sentence
\newcommand{\clause}{\ensuremath{\chi}} % a clause
\newcommand{\term}{\ensuremath{\pi}} % a term
\newcommand{\Val}{\ensuremath{\mathcal{V}}} % set of propositional valuations

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Modal logic:

% Modal operators:
\newcommand{\nec}{\Box}
\newcommand{\poss}{\Diamond}
\newcommand{\Nec}[1]{[ #1 ]}
\newcommand{\Poss}[1]{\langle #1 \rangle}
\newcommand{\obl}{\scalebox{0.75}{\raisebox{0.5ex}{\ensuremath{\bigcirc}}}} % obligation

% Kripke models:
\newcommand{\W}{\ensuremath{\text{\it W}}} % possible worlds
\newcommand{\R}{\ensuremath{\text{\it R}}} % accessibility relation
\newcommand{\V}{\ensuremath{\text{\it V}}} % valuation function
\newcommand{\M}{\mathscr{M}}
\newcommand{\MSet}{\ensuremath{\mathcal{M}}} % set of models
\newcommand{\U}{\mathcal{U}} % set of pointed models

% Modal logic K:
\newcommand{\K}{{\sf K}}
\newcommand{\Ba}{{\sf B}}

\newcommand{\schemaK}{\ensuremath{\text{{\it K}}}}
\newcommand{\ruleRN}{\ensuremath{\text{{\it RN}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Description Logics:

%\newcommand{\CN}{\ensuremath{{\sf N}_{\mathscr{C}}}} % set of concept names
\newcommand{\RN}{\ensuremath{{\sf N}_{\mathscr{R}}}} % set of role names
\newcommand{\Names}{\ensuremath{{\sf N}}}  % union of both (the whole signature)
\newcommand{\dland}{\sqcap}
\newcommand{\dlor}{\sqcup}
\newcommand{\subs}{\sqsubseteq}
\newcommand{\nsubs}{\not\subs}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\Dom}{\Delta}
\newcommand{\ALC}{\ensuremath{\mathcal{ALC}}}
\newcommand{\EL}{\ensuremath{\mathcal{EL}}}
\newcommand{\inv}{^{-}} % for role inverse roles
\newcommand{\ABox}{\ensuremath{\mathcal{A}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special functions and relations:

\newcommand{\atm}[1]{{\ensuremath{\text{\it atm}(#1)}}} % atoms of a sentence
\newcommand{\lit}[1]{{\ensuremath{\text{\it lit}(#1)}}} % literals of a sentence
\newcommand{\sig}[1]{{\ensuremath{\text{\it sig}(#1)}}} % symbols of a sentence
\newcommand{\Mod}[1]{{\ensuremath{\text{\it Mod}(#1)}}} % models of a sentence
\newcommand{\Modrm}[1]{{\ensuremath{\text{\it Mod}_{\mathscr{R}}(#1)}}} % models of a sentence
\newcommand{\Cn}[2]{{\ensuremath{\text{\it Cn}_{#1}(#2)}}} % logical consequence
\newcommand{\pimplicates}[1]{{\ensuremath{\text{\it PI}(#1)}}} % set of prime implicates
\newcommand{\pimplicants}[1]{{\ensuremath{\text{\it IP}(#1)}}} % set of prime implicants
\newcommand{\NC}[2]{{\ensuremath{\text{\it NewCons}(#1,#2)}}} % new consequences

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Nonmonotonic stuff:

% Connectives:
\newcommand{\dimp}{\leadsto}
\newcommand{\ndimp}{\not\dimp}
\newcommand{\twiddle}{\hspace{-0.04cm}\mathrel|\joinrel\sim\hspace{-0.05cm}}
%\newcommand{\twiddle}{ \,\scalebox{1.1}[.9]{$\mathrel{\substack{\textstyle\sqsubset\\[-0.4ex]\scalebox{.8}[.8]{$\textstyle\sim$}}}$}\,}
\newcommand{\ntwiddle}{\mathrel|\joinrel\nsim}
\newcommand{\nmodels}{\mathrel|\joinrel\neq}
\newcommand{\usually}{\raisebox{-0.5ex}{$\:\stackrel{\sqsubset}{{\scriptstyle\sim}}\:$} } 
\newcommand{\nusually}{\not\hspace{-1.1mm}\usually}
\newcommand{\typ}{\bullet}
\newcommand{\typup}[1]{#1^{\typ}}

% Entailment:
\newcommand{\NMentails}{\mathrel|\joinrel\approx}
\newcommand{\nNMentails}{\not\NMentails}
\newcommand{\NMproves}{\mathrel|\joinrel\sim}
\newcommand{\nNMproves}{\not\NMproves}

% Semantic constructions:
\newcommand{\PM}{\mathscr{P}} % preferential model
\newcommand{\RM}{\mathscr{R}} % ranked model
\newcommand{\PI}{\ensuremath{\mathcal{P}}} % preferential DL interpretation
\newcommand{\St}{\ensuremath{\text{\it S}}} % set of states
\newcommand{\lab}{\ensuremath{\ell}} % labeling function
\newcommand{\pref}{\prec} % preference relation
\newcommand{\npref}{\not\pref}
\newcommand{\states}[2]{\llbracket#1\rrbracket^{#2}} % requires package stmaryrd
\newcommand{\rk}{\ensuremath{\text{\it rk}}} % ranking function

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Concrete examples:

\newcommand{\p}{{\sf p}}
\newcommand{\bird}{{\sf b}}
\newcommand{\fly}{{\sf f}}
\newcommand{\ost}{{\sf o}}
\newcommand{\w}{{\sf w}}

\newcommand{\q}{{\sf q}}
\newcommand{\sft}{{\sf t}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Miscellaneous:

% Global options:
\renewcommand{\labelitemi}{{\small\textbullet}}
%\renewcommand\arraystretch{1.5}
%\renewcommand{\familydefault}{\sfdefault} % sets font to sans serif globally 

% Useful commands:
\newcommand{\nil}{\textcolor{white}{a}} 
\newcommand{\todo}[1]{\textcolor{red}{\underline{{\sf #1}}}}

\newcommand{\mathV}{\mathcal{V}}
\newcommand{\mathM}{\mathcal{M}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\imp}{\rightarrow}
\newcommand{\mpref}[1]{\trianglelefteq_{#1}}



\newcommand{\con}{\dotdiv}
\newcommand{\conr}{\barwedge}
\newcommand{\ratcl}{\vDash_{rc}}
\newcommand{\RC}{\ensuremath{\mathcal{RC}}}
\newcommand{\prefcl}{\vDash_{pr}}
\newcommand{\PR}{\ensuremath{\mathcal{P}}}
\newcommand{\fun}{{\sf c}}
\newcommand{\conbpr}{-}
\newcommand{\CN}{\ensuremath{\mathcal{C}}}
\newcommand{\conb}{-}
\newcommand{\prefexp}{+}
\newcommand{\clcon}{-}
\newcommand{\clcont}{-'}
\newcommand{\rev}{*}
\newcommand{\revcoh}{\otimes}
\newcommand{\prefrev}{\bullet}
\newcommand{\prefrevcoh}{\circ}
%\newcommand{\prefexp}{+}


\newcommand{\KBinf}{\ensuremath{\KB^\infty}}
\newcommand{\KBinfAB}{\ensuremath{\KB^\infty}_{A\twiddle\lnot B}}
\newcommand{\KBi}[1]{\ensuremath{\KB^{<\infty}}}
\newcommand{\KBiAB}[1]{\ensuremath{\KB^{<\infty}_{A\twiddle\lnot B}}}
%\newcommand{\KBsinf}[1]{\ensuremath{\text{\raisebox{3pt}{$\scriptscriptstyle{\underset{\infty}{#1}}$}}}}



\newcommand{\Binf}{\ensuremath{\text{\raisebox{3pt}{$\scriptscriptstyle{\underset{\infty}{\B}}$}}}}
\newcommand{\Bi}[1]{\ensuremath{\text{\raisebox{3pt}{$\scriptscriptstyle{\underset{#1}{\B}}$}}}}
\newcommand{\Bsinf}[1]{\ensuremath{\text{\raisebox{3pt}{$\scriptscriptstyle{\underset{\infty}{#1}}$}}}}
\newcommand{\Bsi}[2]{\ensuremath{\text{\raisebox{3pt}{$\scriptscriptstyle{\underset{#2}{#1}}$}}}}


\newcommand{\CL}{\ensuremath{Cn}}
\newcommand{\SCL}[1]{\ensuremath{\text{\raisebox{3pt}{$\scriptscriptstyle{\underset{#1}{\CL}}$}}}}


\newcommand{\CLcontr}{-}
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}

\renewcommand{\sp}{\emph{sp}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RICHARD'S NEWCOMMANDS:

\newcommand{\C}[2]{C_{#1}(#2)}  % specific PTL entailment relations, e.g. \C{\RSet}{\KB} for ranked entailment
\newcommand{\RSet}{\ensuremath{\mathcal{R}}} % set of ranked models
\newcommand{\smpref}[1]{\triangleright_{#1}}
\newcommand{\LM}{\mathrm{LM}}
\newcommand{\rank}[2]{\textit{rank}_{#2}(#1)}

%\newcommand{\kernel}{\ensuremath{\parallel \hspace{-0.32cm}\_\_}}
\newcommand{\remaind}{\ensuremath{\mathbf{\downarrow}}}

\newcommand{\VRBC}{V}
\newcommand{\MRBC}{M}
\newcommand{\ARBC}{A}

\usepackage{xspace}
\usepackage{bussproofs}

\newcommand{\kernel}{\hspace{-0.1cm}\mathbin{\rotatebox[origin=c]{90}{$\models$}}\hspace{-0.1cm}}

